Rotation-Invariant Local-to-Global Representation Learning for 3D Point Cloud

We propose a local-to-global representation learning algorithm for 3D point cloud data, which is appropriate to handle various geometric transformations, especially rotation, without explicit data augmentation with respect to the transformations. Our model takes advantage of multi-level abstraction based on graph convolutional neural networks, which constructs a descriptor hierarchy to encode rotation-invariant shape information of an input object in a bottom-up manner. The descriptors in each level are obtained from a neural network based on a graph via stochastic sampling of 3D points, which is effective in making the learned representations robust to the variations of input data. The proposed algorithm presents the state-of-the-art performance on the rotation-augmented 3D object recognition and segmentation benchmarks, and we further analyze its characteristics through comprehensive ablative experiments.

==> section/6_impact.tex <==
%!TEX root = ./../NIPS.tex
\section*{Broader Impact}
The major goal of our research is to enhance the 3D object recognition by imposing the capability to handle geometric transformation, especially, rotations, effectively.
3D object recognition is applicable to various computer vision systems including autonomous driving, visual surveillance, augmented reality, and many others.
From the societal point of view, the improvement of 3D object recognition algorithms has both bright and dark sides.
These systems can benefit those who are visually impaired by providing assistive vision systems including smart glasses.
Meanwhile, the technology might infringe on personal privacy if equipped in drones and CCTVs.
